Holistic Inverse Rendering of Complex Facade via Aerial 3D Scanning

In this work, we use multi-view aerial images to reconstruct the geometry, lighting, and material of facades using neural signed distance fields (SDFs). Without the requirement of complex equipment, our method only takes simple RGB images captured by a drone as inputs to enable physically based and photorealistic novel-view rendering, relighting, and editing. However, a real-world facade usually has complex appearances ranging from diffuse rocks with subtle details to large-area glass windows with specular reflections, making it hard to attend to everything. As a result, previous methods can preserve the geometry details but fail to reconstruct smooth glass windows or verse vise. In order to address this challenge, we introduce three spatial- and semantic-adaptive optimization strategies, including a semantic regularization approach based on zero-shot segmentation techniques to improve material consistency, a frequency-aware geometry regularization to balance surface smoothness and details in different surfaces, and a visibility probe-based scheme to enable efficient modeling of the local lighting in large-scale outdoor environments. In addition, we capture a real-world facade aerial 3D scanning image set and corresponding point clouds for training and benchmarking. The experiment demonstrates the superior quality of our method on facade holistic inverse rendering, novel view synthesis, and scene editing compared to state-of-the-art baselines.

==> sections/dataset.tex <==

\begin{figure*}[ht]
    \centering
    % \includegraphics[width=\textwidth]{figure/pip_merge.png}
    \includegraphics[width=\textwidth]{figure/pip_v2.pdf}
    \vspace*{-4.5ex}
    % \caption{\textbf{Overview of the pipeline}. On the left, we show that for an incident point $\mathbf{p}$ along with query light direction $\mathbf{d}$, we use screen space ray tracing to trace the source point $\mathbf{s}$ of the query light. The corresponding local feature vector is extracted from feature map $\mathbf{F}$ via projection of point $\mathbf{s}$. The feature is then passed to MLP decoder network $f$ along with light direction and auxiliary G-Buffer information. The output RGB value is compared with the ground truth radiance value. On the right, we show our out-of-view light estimation. We use a hypernetwork to predict the weights of the NeRF MLP and volume render the background lighting.  }
    \caption{\textbf{Overview of the pipeline}. \fl{On the left, we show the workflow throughout our inverse rendering framework: (i) The spatially-varying material and geometry maps are predicted by $\textbf{MGNet}$ (ii) According to the predicted material, geometry and view direction associated with each pixel point $\mathbf{p}$, a BRDF importance sampling is performed to generate per-pixel incident directions $\mathbf{d}_i$ (iii) We use screen-space raytracing to trace the source point $\mathbf{s}$ of the query light. The corresponding local feature vector is extracted from feature map $F$ via projection of point $\mathbf{s}$. (iv) The feature is passed to $\mathbf{LightNet}$ along with light direction and auxiliary G-Buffer information to predict the incident radiance $\tilde{L_i}$ (v) Monte-Carlo integration (Eq.~\ref{equ:render}) is used to calculate the final re-rendered result.} On the right, we show our out-of-view light estimation. We use a hypernetwork to predict the weights of the NeRF MLP and volume render the background lighting.}
    \label{fig:pipeline}
    % \vspace*{-1.\baselineskip}%
\end{figure*}

\section{InteriorVerse: A Large-Scale, Photorealistic Indoor Scene Dataset}
\label{sec:data}
A high-quality dataset is crucial for learning-based inverse rendering. It's extremely difficult to acquire spatially-varying material and lighting ground truth in real world complex indoor scenes. Therefore, we render a synthetic dataset to supervise training. The SUNCG dataset~\cite{song2017semantic} is a manually-created large-scale dataset for indoor scenes, but they use non-physical Phong BRDF and render with OpenGL, which severely limits its photorealism. PBRS~\cite{zhang2017physically} and CG-PBR~\cite{sengupta2019neural} datasets are rendered with physically-based renderers, but both still use Phong BRDF and do not provide spatially-varying lighting ground truth for an arbitrary 3D location. InteriorNet~\cite{li2018interiornet} is a large-scale photorealistic indoor scene dataset providing multiple camera views and panoramas, but the images they provide are LDR, limiting the dynamic range of illumination. OpenRooms~\cite{li2021openrooms} is by far the only HDR dataset with spatially-varying lighting rendered using physically-based microfacet BRDF. However, as shown in Fig.~\ref{fig:dataset}, it presents overly simplified furniture models and layouts, insufficient material and lighting variations, leading to less faithful appearance comparing to real world data consequently.


\begin{figure}[b]
    \centering
    \setlength{\fboxsep}{0.0pt}%
    \setlength{\fboxrule}{0.75pt}%
    \vspace*{-1.0\baselineskip}%
    \hspace*{-0.6ex}%
    \begin{tikzpicture}[x=0.075\textwidth, y=0.075\textwidth,every text node part/.style={align=center}]
    \node[anchor=north west] at (-0.03, 0) {\includegraphics[width=0.155\textwidth]{figure/compare_dataset/open1.png}};
    \node[anchor=north west] at (3.16, 0) {\includegraphics[width=0.155\textwidth]{figure/compare_dataset/ours2.png}};
    
    \node[anchor=north west] at (2.07, 0) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/open2.png}};
    \node[anchor=north west] at (2.07, -0.79+0.0021) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/open4.png}};
    \node[anchor=north west] at (2.07, -1.58) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/open5.png}};
    \node[anchor=north west] at (2.07, -1.58-0.79+0.0021) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/open6.png}};
    
    \node[anchor=north west] at (-0.03, -1.58) {\includegraphics[width=0.155\textwidth]{figure/compare_dataset/open3.png}};
    \node[anchor=north west] at (3.16, -1.58) {\includegraphics[width=0.155\textwidth]{figure/compare_dataset/ours1.png}};
    
    \node[anchor=north west] at (5.26, 0) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/ours4.png}};
    \node[anchor=north west] at (5.26, -0.79+0.0021) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/ours5.png}};
    \node[anchor=north west] at (5.26, -1.58) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/ours6.png}};
    \node[anchor=north west] at (5.26, -1.58-0.79+0.0021) {\includegraphics[width=0.076\textwidth]{figure/compare_dataset/ours7.png}};
 
    \draw[ black, very thin] (3.205,0.18) -- (3.205,-3.218);
    \node at (1.6, 0.08){\textsc{OpenRooms}~\cite{li2021openrooms}};
    \node at (4.8, 0.08){\textsc{InteriorVerse (ours)}};

    \end{tikzpicture}%
    % \vspace*{-1.0\baselineskip}%
    \vspace*{-2.5ex}
    \caption{\textbf{Example dataset images} from OpenRooms~\cite{li2021openrooms} (left) and our \textsc{InteriorVerse} dataset (right). Note that our dataset contains more diversified geometry, material (especially glossy and specular BRDFs) and complex lighting conditions comparing OpenRooms. Zoom in for details.}
    \label{fig:dataset}
    \vspace*{-1.\baselineskip}%
\end{figure}

In this work, we create a new high-quality indoor scene dataset called \textsc{InteriorVerse}, which has the following advantages in data quality over existing alternatives: (1) the scene layouts of our dataset have richer details, including complex furniture and decorations. (2) Our dataset is rendered with GGX BRDF model~\cite{walter2007microfacet}, which has stronger material modeling capability than any BRDF models that existing indoor scene datasets use. (3) Our dataset provides not only pixel-wise surface environment maps, but also contains environment maps located anywhere in the 3D scene space. Fig.~\ref{fig:dataset} compares some example scenes in our dataset and OpenRooms, showing our dataset's higher scene quality.
